EchoPrompt: Instructing the Model to Rephrase Queries for Improved In-context Learning

Language models are achieving impressive performance on various tasks by aggressively adopting inference-time prompting techniques, such as zero-shot and few-shot prompting. In this work, we introduce EchoPrompt, a simple yet effective approach that prompts the model to rephrase its queries before answering them. EchoPrompt is adapted for both zero-shot and few-shot in-context learning with standard and chain-of-thought prompting. Experimental results show that EchoPrompt yields substantial improvements across all these settings for four families of causal language models. These improvements are observed across various numerical reasoning (e.g. GSM8K, SVAMP), reading comprehension (e.g. DROP), and logical reasoning (e.g. Coin Flipping) tasks. On average, EchoPrompt improves the Zero-shot-CoT performance of code-davinci-002 by 5% in numerical tasks and 13% in reading comprehension tasks. We investigate the factors contributing to EchoPrompt's effectiveness through ablation studies, which reveal that both the original query and the model-generated rephrased version are instrumental in its performance gains. Our empirical results indicate that EchoPrompt is an effective technique that enhances in-context learning performance. We recommend incorporating EchoPrompt into various baseline prompting strategies to achieve performance boosts.

==> figures/cond_perp.tex <==
\begin{figure*}[!htb]
\centering
% \begin{subfigure}{0.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/gsm8k_perplex_ltm.png}
%   \caption{GSM8K}
%   \label{fig:sub1}
% \end{subfigure}%
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/svamp_perplex.png}
  \caption{SVAMP}
  \label{fig:sub2}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/drop_census_perplex.png}
  \caption{DROP-Census}
  \label{fig:sub3}
\end{subfigure}
\caption{Violin plots showcasing the conditional perplexity distribution of queries, for SVAMP, and DROP-Census. 
The conditional perplexities of SVAMP are much higher than that of DROP-Census.
Compound Sentence rephrasing reduces the conditional perplexity distribution of the original queries, while Question First rephrasing tends to increase perplexity. 
% Although various factors can influence predictions, conditional perplexity serves as a useful proxy for performance.
}
\label{fig:perplex}
\end{figure*}

==> figures/figure_qrephrase.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
{\promptfont 
\small{
\hlorange{\textbf{[Exemplars]}}\\*
Q: If there are 3 cars in the parking lot and 2 more cars arrive, how many cars are in the parking lot?\\*
A: There are originally 3 cars. 2 more cars arrive. 3 + 2 = 5. The answer is 5.\\*

Q: Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total?\\*
A: Originally, Leah had 32 chocolates. Her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39. The answer is 39.\\*

more exemplars...

Q: \hlorange{\textbf{[Question]}}\\*
A:
}}
        % \caption{chain-of-thought prompting}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.60\textwidth}
{\promptfont 
\small{
\hlorange{\textbf{[Exemplars]}}\\*
Q: If there are 3 cars in the parking lot and 2 more cars arrive, how many cars are in the parking lot?\\*
A: \textred{Rewriting in simple words, the question is: }\hlgreen{"Given that there are currently 3 cars in the parking lot, and 2 more cars arrive, how many cars are in the parking lot now?"}\\*
\textred{Now, to answer the rewritten question, }There are originally 3 cars. 2 more cars arrive. 3 + 2 = 5. The answer is 5.\\*

Q: Leah had 32 chocolates and her sister had 42. If they ate 35, how many pieces do they have left in total?\\*
A: \textred{Rewriting in simple words, the question is: }\hlgreen{"Given that Leah had 32 chocolates and her sister had 42, and they ate a total of 35 pieces, how many pieces of chocolate do they have left in total?"}\\*
\textred{Now, to answer the rewritten question,} Originally, Leah had 32 chocolates. Her sister had 42. So in total they had 32 + 42 = 74. After eating 35, they had 74 - 35 = 39. The answer is 39.\\*

more exemplars...

Q: \hlorange{\textbf{[Question]}}\\*
A:
}}
        % \caption{chain-of-thought prompting with query rephrasing subtask}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
        \caption{Query-Rephrasing as a subtask. The language model is guided to rephrase the original problem in a specific structure by being presented with exemplars that showcase this structure. By exposing the model to such exemplars, it gains insights into the significance of Query-Rephrasing subtask before attempting its solution. This approach enhances the model's capacity to recall and reconstruct a version of the original query, thereby strengthening its comprehension of the query at hand.}
        \label{figure:qrephrase}
\end{figure*}

==> tables/acc_by_steps.tex <==
\begin{table}[tb]
  \centering
  \small
    \begin{tabular}{llllll}
  \toprule
      Approach & 2 & 3 & 4 & 5 & >=6  \\ \midrule
      \textbf{GSM8K} \\ 
      CoT & 77.3 & 67.6 & 56.5 & 51.2 & 29.1  \\ 
      CoT+ Compound & \textbf{84.3} & \textbf{71.8} & \textbf{60.8} & 55.2 & \textbf{36.4} \\ 
      
      LTM & 78.8 & 68.3 & 57.8 & \textbf{55.7} & 30.4 \\ \addlinespace
      
      \textbf{DROP (break)}\\ 
      CoT & N/A & 66.7 & 56.9 & 60.5 & 76.3  \\ 
      CoT+Compound & N/A & \textbf{70.4} & 59.8 & \textbf{67.2} & \textbf{79.3} \\ 
      LTM & N/A & 61.7 & \textbf{63.2} & 60.5 & 71.8  \\ \bottomrule
  \end{tabular}
  \caption{\textbf{code-davinci-002} Comparision of accuracies of \echoprompt{}, chain-of-thought(CoT) and least-to-most(LTM) prompting broken down by the number of reasoning steps required in the expected solution. \echoprompt{} outperforms both CoT and LTM.}
  \label{table:acc_by_steps}
\end{table}

==> tables/acc_by_steps_ltm.tex <==
% \begin{table*}[!ht]
%   \centering
%   \begin{tblr}{
%     colspec={X[1.75]X[2.5]XXXXX}, row{1} = {l},
%   }
%   \hline
%       \textbf{Dataset} & \textbf{Approach} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{>=6} \\ \hline
%       GSM8K & COT\small{(LTM)} & 81.60 & 71.35 & 61.87 & 60.34 & 41.72 \\ 
%       ~ & COT\small{(LTM)}+QRefine\small{(best)} & 81.90 & 72.78 & 68.9 & 61.92 & 43.04 \\ 
%       ~ & LTM & 81.90 & 74.05 & 60.2 & 62.64 & 41.06 \\ \hline
%       DROP \small{(break)} & COT(LTM) & 38.89 & 74.21 & 63.19 & 70.15 & 78.28 \\ 
%       ~ & COT\small{(LTM)}+Refine\small{(best)} & 50 & 72.33 & 69.44 & 71.64 & 78.28 \\ 
%       ~ & LTM & 38.89 & 64.15 & 63.19 & 59.7 & 73.23 \\ \hline  
%       \end{tblr}
%   \caption{Accuracy by Steps COT LTM prompts}
% \end{table*}


\begin{table*}[!ht]
  \centering
  \small
  \begin{tabular}{lllllll}
  \toprule
     % &  & Prompts tailored to CoT & & & & & Prompts tailored to LTM &  &  & & \\
      Dataset & Approach & 2 & 3 & 4 & 5 & >=6 \\ \midrule
      GSM8K & COT & 81.3 & 71.1 & 62.2 & 61.5 & 39.7  \\ 
      ~ & CoT+Compound & \textbf{84.3} & 72.4 & \textbf{67.2}  & \textbf{64.9} & 39.8\\ 
      ~ & LTM & 81.9 & \textbf{74.1} & 60.2 & 62.6 & \textbf{41.1} \\ \midrule
      
      DROP  & COT &  N/A & \textbf{74.2} & 63.2 & 69.4 & 77.3 \\ 
      \small{(break)} & CoT+Compound &  N/A & 71.1 & \textbf{66.7} & \textbf{71.6} & \textbf{78.8} \\ 
      ~ & LTM & N/A & 62.9 & 63.2 & 60.5 & 72.7 \\ \bottomrule
  \end{tabular}
  \caption{\textbf{Code-davinci-002: Accuracy with number of reasoning steps} This table presents the analysis of \echoprompt{'s} performance on GSM8K and DROP (break subset) datasets. The queries in these datasets are categorized based on the number of reasoning steps required to solve them. Exemplars demonstrating longer chain-of-thought reasoning were used for evaluation. \echoprompt{} showcases improvements across all ranges of reasoning steps.}
  \label{table:acc_by_steps_ltm}
\end{table*}





==> tables/cot_ltm.tex <==
% \begin{table*}[!ht]
%   \centering
%   \begin{tblr}{
%     colspec={X[2.3]XXXXXX}, row{1} = {l},
%   }
%   \hline
%       \textbf{} & \textbf{GSM8K} & \textbf{SVAMP} & \textbf{ASDIV} & \textbf{\makecell[tl]{DROP \\ \small{(football)}}} & \textbf{\makecell[tl]{DROP \\ \small{(non-football)}}} & \textbf{\makecell[tl]{DROP \\ \small{(break)}}} \\ \hline
%       % Baseline CoT & - & - & - & 59.6 & 74.77 & - \\ 
%       Standard & 17.12 & 67.70 & 67.50 & 63.71 & 60.53 & 56.72 \\
%       Standard+QRephrase & \textbf{18.86} & \textbf{72.00} & \textbf{70.41} & \textbf{67.89} & \textbf{65.91} & \textbf{63.15}\\ \hline
%       CoT & 66.89 & 74.70 & 75.05 & 67.33 & 75.9 & 70.63 \\ 
            
%       \makecell[tl]{CoT+QRephrase\small{(best)}} & \textbf{69.47} & 76.50 & 75.2 & \textbf{72.01} & 77.3 & \textbf{72.48} \\ 
      
%       \makecell[tl]{CoT+QRepeat} & 68.2 & 75.30 & \textbf{75.75} & 71.06 & \textbf{78.1} & 72.01 \\ 
%       LTM & 67.57 & \textbf{79.60} & 74.57 & 66.23 & 73.32 & 65.29 \\ \hline
%   \end{tblr}
%   \caption{code-davinci-002 CoT LTM Prompts}
%   \label{figure:codex:ltm}
% \end{table*}


==> tables/cot_turbo.tex <==
% \begin{table*}[!ht]
%     \centering
%     \begin{tblr}{
%       colspec={X[2]X[3.5]|XXXXX}, row{1} = {l},
%     }
%     \hline
%     \textbf{\small{Method}} & \textbf{\small{Stage-1 Prompt}} & \textbf{\small{GSM8K}} & \textbf{\small{SVAMP}} & \textbf{\small{DROP(break)}} & \textbf{\small{Date\footnote{The task setup is different from \citep{kojima2022large}. The previous work treats the task as a multiple choice question.}}} \\
%     \hline
%     Zero-shot & - & 55.07 & 51.90 & 45.11 & 35.77 \\
%     Zero-shot+ QRephrase & Let's repeat the complete question. `` & - & 76.0 & 42.2 & 31.16 \\ \hline

%     Zero-shot-CoT & Let's think step by step. & 75.91 & 80.50 & 53.37 & 47.15 \\
%     & Let's repeat the complete question and also think step by step. & 76.87 & 79.68 & 46.58  & 51.27 \\ 
%     \hline
%     \end{tblr}
%     \caption{Zero-shot results GPT-3.5-Turbo}
%     \label{table:zeroshot-turbo}
% \end{table*}







% \begin{table*}[!ht]
%   \centering
%   \begin{tblr}{
%     colspec={X[2]XXX[1.5]XXX}, row{1} = {l},
%   }
%   \hline
%       % \textbf{} & \textbf{GSM8K} & \textbf{SVAMP} & \textbf{DROP(break)} & \textbf{SCAN \\\small{(500 samples)}} & \textbf{SQuADv2 \\\small{(500 samples)}} & \textbf{Date} \\ \hline
% \textbf{} & \textbf{GSM8K} & \textbf{SVAMP} & \textbf{DROP(break)} & \textbf{SCAN} & \textbf{SQuAD(F1)} & \textbf{Date} \\ \hline
%       Standard  & 31.31 & 76.1 & 59.94 & 4.60 & 76.42 & 50.40 \\
      
%       Standard+QRephrase & 32.14 & 78.4 & 62.69 & 1.60 & 83.22 & 48.34 \\ \hline
      
%       CoT                & 75.07 & 77.4 & 61.62 & 15 & 83.12 & 64.49 \\ 
      
%       \makecell[tl]{CoT+QRephrase\small{(best)}} & 82.57 & 80.7 & 66.51 & 13.4 & 83.75 & 66.12 \\ 
      
%       CoT+QRepeat & 83.48 & 81.9 & 63.8 & - & - & 64.8 \\ 
%   \end{tblr}
  
%   \caption{Turbo-3.5}
%   \label{figure:fewshot-turbo}
% \end{table*}



% \begin{table*}[!ht]
%   \centering
%   \small
%   \begin{tblr}{
%     colspec={X[3,c]|X[1,c]X[1.5,c]|X[1,c]X[1.5,c]|X[1,c]X[1.5,c]|X[1,c]X[1.5,c]}, row{1} = {c},
%     cell{1}{2} = {c=4}{c},
%     cell{1}{6} = {c=4}{c},
%     cell{1}{1} = {r=2}{c},
%     cell{2}{2,4,6,8} = {c=2}{c}
%   }   
  
%   \hline
%   & \small\textbf{Zero-shot} &  &  &  & \small\textbf{Few-shot} & & &  \\\hline
%   & \small{Standard} & & \small{CoT} &  & \small{Standard} &  & \small{CoT} &\\\hline
%   \small{\echoprompt{} ?} & \large{\xmark} & \large{\cmark} & \large{\xmark} & \large{\cmark}   & \large{\xmark}  & \large{\cmark}  & \large{\xmark}  & \large{\cmark}  \\
%   \hline
% GSM8K & 5.6 & 24.8\deltadiff{19.2} & 75.7 & 76.4\deltadiff{0.7} & 31.3 & 32.1\deltadiff{0.8} & 75.1 & 83.5\deltadiff{8.4} \\
% SVAMP & 51.9 & 76.0\deltadiff{24.1} & 80.5 & 79.7\deltadiff{-0.8} & 76.1 & 78.4\deltadiff{2.3} & 77.4 & 81.9\deltadiff{5.5} \\
% Date & 33.6 & 46.6\deltadiff{13} & 47.1 & 51.3\deltadiff{4.2} & 50.4 & 48.3\deltadiff{-2.1} & 64.5 & 66.2\deltadiff{1.7} \\
% \hline
% \makecell[tl]{DROP\small{(Break)}} & 47.1 & 46.4\deltadiff{-0.7} & 53.4 & 45.6 & 59.9 & 62.7\deltadiff{2.8} & 61.6 & 66.5\deltadiff{4.9} \\
% SQuAD(F1) & 79.1 & 80.6\deltadiff{1.5} & - & - & 76.4 & 83.2\deltadiff{6.8} & - & - \\ \hline  
%   \end{tblr}
% \caption{\textbf{GPT-Turbo-3.5:} GPT-3.5-Turbo exhibits superior numerical and logical reasoning capabilities, although it slightly lags in zero-shot reasoning. Notably, \echoprompt{} technique improves the performance on most of the tasks.}
% \label{table:turbo}
% \end{table*}


\begin{table*}[!ht]
  \centering
  \small
  \begin{tabular}{l|ll|ll|ll|ll}
    \hline
    & \multicolumn{4}{c|}{Zero-shot} & \multicolumn{4}{c}{Few-shot}  \\ 
    \cline{2-9}
    & \multicolumn{2}{c}{Standard} & \multicolumn{2}{c|}{CoT} & \multicolumn{2}{c}{Standard} & \multicolumn{2}{c}{CoT}  \\ \hline
    % \echoprompt{} ? & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark \\ \hline
    \echoprompt{} ? & \multicolumn{1}{c}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c}{\xmark} & \multicolumn{1}{c}{\cmark} \\ \hline
    GSM8K & 5.6 & 24.8\deltadiff{19.2} & 75.7 & 76.4\deltadiff{0.7} & 31.3 & 32.1\deltadiff{0.8} & 75.1 & 83.5\deltadiff{8.4} \\
    SVAMP & 51.9 & 76.0\deltadiff{24.1} & 80.5 & 79.7\deltadiff{-0.8} & 76.1 & 78.4\deltadiff{2.3} & 77.4 & 81.9\deltadiff{5.5} \\
    Date & 33.6 & 46.6\deltadiff{13} & 47.1 & 51.3\deltadiff{4.2} & 50.4 & 48.3\deltadiff{-2.1} & 64.5 & 66.2\deltadiff{1.7} \\ \hline
    DROP\small{(Break)} & 47.1 & 46.4\deltadiff{-0.7} & 53.4 & 45.6 & 59.9 & 62.7\deltadiff{2.8} & 61.6 & 66.5\deltadiff{4.9} \\
    SQuAD(F1) & 79.1 & 80.6\deltadiff{1.5} & - & - & 76.4 & 83.2\deltadiff{6.8} & - & - \\ \hline
  \end{tabular}
  \caption{\textbf{GPT-Turbo-3.5:} GPT-3.5-Turbo exhibits superior numerical and logical reasoning capabilities, although it slightly lags in zero-shot reasoning. Notably, \echoprompt{} technique improves the performance on most of the tasks.}
  \label{table:turbo}
\end{table*}


==> tables/gptjmodels.tex <==
% \begin{table*}[!htb]
%   \centering
%   \begin{tblr}{
%     colspec={X[1.5]XX[1.5]XXX|X}, row{1} = {l},
%   }

%   \hline
%       Model & & \echoprompt{} & Coin Flip & SVAMP & ASDiv & Date  \\ \hline
      
%   Starcoder-15B & Standard   & - & 98.6 & 32.4 & 34.0 & 24.4\\
%   ~ & & Rephrase \small{(best)} & 100.0\deltadiff{1.4} & 36.7\deltadiff{4.3} & 34.8\deltadiff{0.8} & 25.2\deltadiff{0.8}  \\
%   ~ &  & Repeat & 99.8\deltadiff{1.2} & 37.2\deltadiff{4.8} & 36.8\deltadiff{2.8} & 26.6\deltadiff{2.2} \\
  
%    & CoT & - & 100.0& 31.6 & 36.0 & 37.7  \\
%   ~ & & Rephrase \small{(best)} & 100.0\deltadiff{0} & 29.9\deltadiff{-1.7} & 36.4\deltadiff{0.4} & 30.9\deltadiff{-6.8}  \\
%   ~ & & Repeat & 100.0\deltadiff{0} & 33.3\deltadiff{1.7} & 37.2\deltadiff{1.2} & 27.9\deltadiff{-9.8}  \\ \hline


%   Llama-13B & Standard & - & 89.8 & 39.2 & 43.8 & 32.8  \\
%   ~ & & Rephrase \small{(best)} & 98.7\deltadiff{8.9} & 44.9\deltadiff{5.7} & 46.5\deltadiff{2.7}  & 32.2\deltadiff{-0.6}  \\
%   ~ & & Repeat & 92.7\deltadiff{2.9} & 43.0\deltadiff{3.8} & 44.6\deltadiff{0.8} & 30.1 \deltadiff{1.7}  \\
%   ~ & CoT & - & 100.0 & 37.7 & 49.2 & 42.3  \\
%   ~ & & Rephrase \small{(best)} & 100.0\deltadiff{0} & 35.4\deltadiff{-2.3} & 48.5\deltadiff{-0.7} & 40.4\deltadiff{-1.9}  \\
%   ~ & & Repeat & 100.0\deltadiff{0} & 34.7\deltadiff{-3.0} & 48.7 \deltadiff{-0.5} & 41.2\deltadiff{-1.1}  \\ \hline
  
%   GPT-J-6B & Standard & - & 81.3 & 8.9 & 11.2 & 13.2  \\ 

  
%   ~ & & Rephrase \small{(best)} & \textbf{81.8}\deltadiff{0.5} & 10.1\deltadiff{1.2} & 14.1\deltadiff{2.9} & \textbf{14.1}\deltadiff{0.9}  \\

%   ~ & & Repeat & 81.3\deltadiff{0} & 9.5\deltadiff{0.6} & 12.8\deltadiff{1.6} & 13.6\deltadiff{0.4}  \\ 
  
%    & CoT & - & 80.6 & 21.1 & 21.3 & 11.1  \\ 
   
%   ~ & & Rephrase \small{(best)} & \textbf{96.4}\deltadiff{15.8} & 19.8 & 19.8\deltadiff{-1.5} & \textbf{15.8}\deltadiff{4.7}  \\
  
%   ~ & & Repeat & 88.6\deltadiff{8.0} & 18.6 & 22.2\deltadiff{0.9} & 15.2\deltadiff{4.1}  \\ \hline
%   \end{tblr}
%   \caption{\textbf{Starcoder-15B, Llama-13B, GPT-J-6B:} \echoprompt{} improves performance on standard prompting, while the results are inconsistent for chain-of-thought prompting.}
%   \label{table:gptmodels}
% \end{table*}

\begin{table*}[!hbt]
  \centering
  \small
  \begin{tabular}{llllllll}
  \toprule
      Model &  & \echoprompt{} & Coin Flip & SVAMP & ASDiv & Date & SingleOp \\ \midrule
  % Starcoder-15B & Standard & & & & \\
  Starcoder-15B & Standard & - & 98.6 & 32.4 & 34.0 & 24.4 & 64.0 \\
  & ~ &Rephrase \small{(best)} & \textbf{100.0}\deltadiff{1.4} & 36.7\deltadiff{4.3} & 34.8\deltadiff{0.8} & 25.2\deltadiff{0.8} & 68.6\deltadiff{4.6}  \\
  & ~ & Repeat & 99.8\deltadiff{1.2} & \textbf{37.2}\deltadiff{4.8} & \textbf{36.8}\deltadiff{2.8} & \textbf{26.6}\deltadiff{2.2} & 70.1\deltadiff{6.1} \\ \hdashline
  % & CoT & & & & \\
  & CoT & - & 100.0& 31.6 & 36.0 & \textbf{37.7} &  \\
  & ~ & Rephrase \small{(best)} & 100.0\deltadiff{0.0} & 29.9\deltadiff{-1.7} & 36.4\deltadiff{0.4} & 30.9\deltadiff{-6.8} &  \\
  & ~ & Repeat & 100.0\deltadiff{0.0} & \textbf{33.3}\deltadiff{1.7} & \textbf{37.2}\deltadiff{1.2} & 27.9\deltadiff{-9.8} & \\ \addlinespace \midrule
  % Llama-13B & Standard & & & & \\
   Llama-13B & Standard & - & 89.8 & 39.2 & 43.8 & \textbf{32.8} & 81.1 \\
  & ~ & Rephrase \small{(best)} & \textbf{98.7}\deltadiff{8.9} & \textbf{44.9}\deltadiff{5.7} & \textbf{46.5}\deltadiff{2.7}  & 32.2\deltadiff{-0.6}  & 82.7\deltadiff{1.6}\\
  & ~ & Repeat & 92.7\deltadiff{2.9} & 43.0\deltadiff{3.8} & 44.6\deltadiff{0.8} & 30.1 \deltadiff{-1.7} & \textbf{83.3}\deltadiff{2.2}  \\ \hdashline
  % & CoT & & & & \\
  & CoT  & - & 100.0 & \textbf{37.7} & \textbf{49.2} & \textbf{42.3}  \\
  & ~ & Rephrase \small{(best)} & 100.0\deltadiff{0.0} & 35.4\deltadiff{-2.3} & 48.5\deltadiff{-0.7} & 40.4\deltadiff{-1.9}  \\
  & ~ & Repeat & 100.0\deltadiff{0.0} & 34.7\deltadiff{-3.0} & 48.7 \deltadiff{-0.5} & 41.2\deltadiff{-1.1}  \\ \addlinespace \midrule
  % GPT-J-6B & Standard & & & & \\
   GPT-J-6B & Standard & - & 81.3 & 8.9 & 11.2 & 13.2  & 37.2 \\ 
  & ~ & Rephrase \small{(best)} & \textbf{81.8}\deltadiff{0.5} & \textbf{10.1}\deltadiff{1.2} & \textbf{14.1}\deltadiff{2.9} & \textbf{14.1}\deltadiff{0.9} & 38.8\deltadiff{1.6} \\
  & ~ &Repeat & 81.3\deltadiff{0.0} & 9.5\deltadiff{0.6} & 12.8\deltadiff{1.6} & 13.6\deltadiff{0.4} & \textbf{39.9}\deltadiff{2.7}  \\ \addlinespace \hdashline
    % &  & CoT & & & & \\
  & CoT & - & 80.6 & \textbf{21.1} & 21.3 & 11.1  \\ 
  & ~ & Rephrase \small{(best)} & \textbf{96.4}\deltadiff{15.8} & 19.8\deltadiff{-1.3} & 19.8\deltadiff{-1.5} & \textbf{15.8}\deltadiff{4.7}  \\
  & ~ &Repeat & 88.6\deltadiff{8.0} & 18.6\deltadiff{-2.5} & \textbf{22.2}\deltadiff{0.9} & 15.2\deltadiff{4.1}  \\ \bottomrule
  \end{tabular}
  \caption{\textbf{Starcoder-15B, Llama-13B, GPT-J-6B:} \echoprompt{} improves performance on standard prompting, while the results are inconsistent for chain-of-thought prompting.}
  \label{table:gptmodels}
\end{table*}

